FABULA: Intelligence Report Generation Using Retrieval-Augmented Narrative Construction

Narrative construction is the process of representing disparate event information into a logical plot structure that models an end to end story. Intelligence analysis is an example of a domain that can benefit tremendously from narrative construction techniques, particularly in aiding analysts during the largely manual and costly process of synthesizing event information into comprehensive intelligence reports. Manual intelligence report generation is often prone to challenges such as integrating dynamic event information, writing fine-grained queries, and closing information gaps. This motivates the development of a system that retrieves and represents critical aspects of events in a form that aids in automatic generation of intelligence reports. We introduce a Retrieval Augmented Generation (RAG) approach to augment prompting of an autoregressive decoder by retrieving structured information asserted in a knowledge graph to generate targeted information based on a narrative plot model. We apply our approach to the problem of neural intelligence report generation and introduce FABULA, framework to augment intelligence analysis workflows using RAG. An analyst can use FABULA to query an Event Plot Graph (EPG) to retrieve relevant event plot points, which can be used to augment prompting of a Large Language Model (LLM) during intelligence report generation. Our evaluation studies show that the plot points included in the generated intelligence reports have high semantic relevance, high coherency, and low data redundancy.

==> evaltable4.tex <==
\begin{table*}[ht]
\footnotesize
\centering
\begin{tabular}{|lll|}
\hline
\multicolumn{3}{|c|}{\textbf{2018 Taiwan-China Disinformation Propaganda}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Prompt Template}} & \multicolumn{1}{c|}{\textbf{Prompt}} & \multicolumn{1}{c|}{\textbf{Generated Text}} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Lead Template\\ \textless{}$p_{who}$, $p_{what}$, \\ $p_{when}$, $p_{where}$,\textgreater{}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textless{}Su Chi-cheng, China, Consulate, Taiwanese, fake news, \\ Wednesday, Sept. 4, Taiwanese could be evacuated if they \\ identified themselves as ``Chinese'', stranded travelers could \\ take airport buses to nearby Izumisano Station, \\ where they could board trains \textgreater{}\end{tabular}} & \begin{tabular}[c]{@{}l@{}} Su Chi-cheng allegedly committed suicide \\ due to deep rooted Chinese disinformation campaigns \\ targeting Taiwainese nationals. On Wednesday, Sept. 4. \\ Taiwanese evacuation was only possible if labeled \\ ``Chinese''. The Chinese consulate in Osaka, Japan, \\ said it was aware of the situation and was \\ working to help stranded travelers at Izumisano. \\ The consulate said it was working to provide \\ information to the public \\ and to the media. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Body Template\\ \textless{}$p_{evidence}$, \\ $p_{quote}$,\textgreater{}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textless{} Some social media reports said that Taiwanese citizens … \\ feign Chinese identities, seat on evacuation buses, Death by \\ suicide of Su Chi-cheng…Sept. 14 … criticism aimed at his \\ consulate halted, Su’s death … major examples of Internet \\ disinformation efforts by the Chinese government had \\ real-world consequences,``mother country'' is so powerful'', \\ foreigners trapped … Kansai International Airport are stupid, \\ Japanese airport authorities arranged evacuation buses … \\ Chinese consulate allegedly arranged its own transport to \\ rescue others. The story was later confirmed to be fake \\ when a Taiwanese traveler…confirmed that outside buses \\ could not enter the airport’s pickup area … bridge to the airport … \\ closed to outside traffic.
\textgreater{}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}
The Chinese government has been accused of using social \\ media to spread disinformation and propaganda about \\ Su Chi-cheng. The incident occurred at the \\ Kansai International Airport  where the airport \\ authority said it had arranged for the evacuation \\ of all passengers, regardless of nationality, \\ and that the Chinese consulate had arranged its own \\ transport to rescue their own people, leaving the Taiwanese \\ nationals stranded in Japan. However, the story was \\ debunked when a Taiwanese traveler revealed that outside \\ buses couldn't enter due to the damaged bridge \\ leading to the airport. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Tail Template\\ \textless{}$p_{tactic}$,\textgreater{}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textless{} It is not improbable, then, that the KMT is attempting to \\ preemptively counter accusations that it is benefiting from \\ Chinese disinformation efforts by accusing the DPP, The incident \\ begs series reflection on the collective psychological stress \\ that stems from years of political tension between China and Taiwan.\textgreater{} \end{tabular}} & The KMT is enforcing political tension between China and Taiwan.  \\ \hline
\multicolumn{3}{|c|}{\textbf{2023 Canadian Wildfire Misinformation}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Prompt Template}} & \multicolumn{1}{c|}{\textbf{Prompt}} & \multicolumn{1}{c|}{\textbf{Generated Text}} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Lead Template\\ \textless{}$p_{who}$, $p_{what}$, \\ $p_{when}$, $p_{where}$,\textgreater{}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textless{}Americans, wildfire, smoke, US, Canada, Northeast, Quebec, \\ pollution, pollution, respiratory disease, coordinated attack \\ satellite images, ignitions, social media, footage, June 2, \\ The conditions that caused Canada’s extreme wildfires … \\ resulted in parts of the US and Canada to be \\ blanketed in toxic smoke\textgreater{}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}  Millions of Americans are in public health risk caused by \\ extreme levels of wildfire smoke sourced from \\ Quebec Canada’s wildfires caused toxic smoke, \\ igniting US and Canada which occurred on June 2. \end{tabular} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Body Template\\ \textless{}$p_{evidence}$, \\ $p_{quote}$,\textgreater{}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textless{} The 2023 Canadian wildfire season has been the largest \\ and most devastating, on record, with nearly 14m hectares \\ burned, an area larger than Greece, Posts on social media, \\ have shared a clip speeding through this satellite footage \\ to claim it shows that the fires started ``all at once'' \\ and that this is evidence of a “coordinated attack”, \\ speculated the cause of the fires could have been \\ due to coordinated activity or a large scale, targeted attack, \\ Viral video of satellite images is not evidence that \\ Quebec fires were orchestrated attacks, \\ Video footage shows helicopters dropping \\ flames and embers on trees in Canada.\textgreater{}\end{tabular}} & \begin{tabular}[c]{@{}l@{}} The 2023 Canadian wildfire season is the largest on record \\ with 14m hectares burned. Social media posts claim a \\ satellite clip shows the fires starting ``all at once'' \\ as evidence of a coordinated attack. However, this \\ viral video is not proof of orchestrated attacks. Satellite \\ images and radar footage shared on social media \\ claim that the wildfires were caused by a coordinated attack \\ inspired by orchestrated ignitions. 
\end{tabular} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Tail Template\\ \textless{}$p_{tactic}$,\textgreater{}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textless{}Conclusion: Misleading. A video depicting satellite images \\ of Quebec shows existing fires quickly growing \\ due to documented weather conditions. \\ It is not evidence of a coordinated attack as claimed online.\textgreater{}\end{tabular}} & \begin{tabular}[c]{@{}l@{}} The coordinated activity posted live videos of helicopters \\ dropping flames in Canada. Quebec fires intensified  \\ due to weather conditions, not a coordinated attack.




\end{tabular} \\ \hline
\end{tabular}
\label{tab:generatedtextsamples}
\vspace{2mm}
\caption{Guided autoregressive narrative construction using IPP prompt templates.}
\vspace{-7mm}
\end{table*}
